Mapping the Potential of Explainable AI for Fairness Along the AI Lifecycle

The widespread use of artificial intelligence (AI) systems across various domains is increasingly surfacing issues related to algorithmic fairness, especially in high-stakes scenarios. Thus, critical considerations of how fairness in AI systems might be improved -- and what measures are available to aid this process -- are overdue. Many researchers and policymakers see explainable AI (XAI) as a promising way to increase fairness in AI systems. However, there is a wide variety of XAI methods and fairness conceptions expressing different desiderata, and the precise connections between XAI and fairness remain largely nebulous. Besides, different measures to increase algorithmic fairness might be applicable at different points throughout an AI system's lifecycle. Yet, there currently is no coherent mapping of fairness desiderata along the AI lifecycle. In this paper, we we distill eight fairness desiderata, map them along the AI lifecycle, and discuss how XAI could help address each of them. We hope to provide orientation for practical applications and to inspire XAI research specifically focused on these fairness desiderata.

==> Copyright-logo.tex <==
CEUR-WS Restricted Use Logo License
Copyright (c) 2020 CEUR-WS.org Team

1. The CEUR-WS logo is reserved for use at CEUR-WS.org. Please do not use the CEUR-WS logo on your website.
2. The CEUR-WS logo can be used in the official template for publishing articles on CEUR-WS.
3. We reserve the right to revoke a license for the CEUR-WS logo.


==> content/01_intro.tex <==
\section{Introduction}
\label{sec:intro}



==> content/save.tex <==
\section{Lifecycle}

The progression of methodologies for developing and managing AI applications in general and machine learning (ML) applications in specific is marked by significant contributions over the years, starting with foundational frameworks and evolving to address the comprehensive lifecycle. Initially, the KDD Process introduced in 1996 laid the groundwork for knowledge discovery in databases, offering early insights into the systematic extraction of valuable information from large datasets \cite{fayyad1996data}. Building upon these foundational concepts, \citeauthor{Wirth2000CrispdmTA}~\cite{Wirth2000CrispdmTA}~proposed the CRISP-DM framework, a structured methodology that guides through six critical stages: 1) understanding the business context, 2) grasping the data, 3) preparing the data, 4) modeling, 5) evaluating, and 6) finally deploying the solution. Despite its comprehensive approach, CRISP-DM left the post-deployment phase---and, therefore, human interaction with the systems---largely unexplored. The discourse on the lifecycle of ML applications was further advanced by \citeauthor{wang2017machine}~\cite{wang2017machine}, who emphasized the iterative nature of ML development and the vital role of feedback loops for continuous refinement as well as a focus on the deployment step. Following this, \citeauthor{quemy2020two}~\cite{quemy2020two} delved into the operational challenges inherent to ML systems, advocating for agile and adaptable methodologies that accommodate the fluid dynamics of ML projects. Concurrently, \citeauthor{kuhl2021conduct}~\cite{kuhl2021conduct} provided an in-depth analysis of lifecycle management challenges in information systems research, calling for rigorous documentation of such projects.

\citeauthor{Amershi2019}~\cite{Amershi2019} addressed the post-deployment gap in the CRISP-DM framework by introducing a model that extends the ML lifecycle to include post-deployment activities, thus offering a more holistic view of ML system management. Further enriching this landscape, CRISP-ML(Q) \cite{Studer2021CRISPMLQ} expanded upon CRISP-DM by incorporating a monitoring and maintenance phase, coupled with a detailed quality assessment for each stage and task, thereby emphasizing the need for ongoing oversight and evaluation post-deployment.

Most recently, the MLOps framework by \citeauthor{Kreuzberger2023MLOPS}~\cite{Kreuzberger2023MLOPS} provided an exhaustive exploration of the essential tasks and competencies required for the sustainable development and maintenance of ML applications beyond their initial rollout from a DevOps perspective. This framework underscores the significance of a comprehensive approach that spans the entire lifecycle of ML systems, from conception through to ongoing management and optimization.

Collectively, these contributions illustrate the evolving understanding and methodologies in the field of AI application development and lifecycle management, highlighting a shift towards frameworks that encompass the full spectrum of activities, including those crucial post-deployment phases. We summarize these insights into the AI lifecycle (see \Cref{fig:lifecycle}).


\section{Fairness Mapping Along the AI Lifecycle Remains Incomplete}

Prior works have mapped different fairness considerations to dimensions of the AI lifecycle.
\citet{fazelpour2021algorithmic} map different forms of algorithmic biases along the algorithm pipeline, starting with biases related to  \emph{1) problem specification}.
These involve considerations related to the goals that an algorithm is intended to achieve.
Herein, unfairness might arise when specifying a certain target variable has differential impacts on demographic groups~\citep{obermeyer2019dissecting}.
Moreover, the very choice using AI to (semi-)automate certain decisions may be considered unfair~\citep{barocas-hardt-narayanan}, and has been argued to alter societal values~\citep{merry2016seductions}.

\citet{fazelpour2021algorithmic} then move on to discussing biases that arise during \emph{2) data collection and pre-processing}.
A helpful distinction to make here is between biases that stem from collecting data from biased systems versus biases in the data collection process itself~\cite{ijcai2017p654,mitchell2021algorithmic}.
For instance, if we collect data from a university where systemic racism is detrimentally affecting success of minority groups, training standard supervised machine learning models based on such data will likely lead to perpetuating these harmful structural biases~\citep{fazelpour2021algorithmic}.
This is often referred to as ``bias in, bias out''~\cite{mayson2018bias}.
On the other hand, independently of existing structural biases in systems, we can introduce harmful biases through biased measurement methods~\citep{fazelpour2021algorithmic}, such as using non-representative input data---which may result in algorithms under-performing on minority groups~\citep{buolamwini2018gender}---or training a model on biased labels, such as historical human decisions~\cite{schoeffer2021ranking}.


, then moving on to  , (iii) \textit{modeling and validation}, and finally (iv) \textit{deployment}.

\citet{de2022algorithmic}

\citet{calegari2023assessing}

\citet{li2023trustworthy}

\citet{du2020fairness} also talk about interpretability for fairness

\citet{amugongo2023operationalising}

Health context: \citet{dankwa2021proposed}

Bias: \citet{lee2021risk,singh2022fair,agarwal2023seven}

Toolkits: \citet{bellamy2019ai}

Discuss the pre-, in-, and post-processing proposals.

Problem that some of our identified notions of fairness are not mapped in existing frameworks (?)
